Bayesian Persuasion for Algorithmic Recourse

When subjected to automated decision-making, decision subjects may strategically modify their observable features in ways they believe will maximize their chances of receiving a favorable decision. In many practical situations, the underlying assessment rule is deliberately kept secret to avoid gaming and maintain competitive advantage. The resulting opacity forces the decision subjects to rely on incomplete information when making strategic feature modifications. We capture such settings as a game of Bayesian persuasion, in which the decision maker offers a form of recourse to the decision subject by providing them with an action recommendation (or signal) to incentivize them to modify their features in desirable ways. We show that when using persuasion, the decision maker and decision subject are never worse off in expectation, while the decision maker can be significantly better off. While the decision maker's problem of finding the optimal Bayesian incentive-compatible (BIC) signaling policy takes the form of optimization over infinitely-many variables, we show that this optimization can be cast as a linear program over finitely-many regions of the space of possible assessment rules. While this reformulation simplifies the problem dramatically, solving the linear program requires reasoning about exponentially-many variables, even in relatively simple cases. Motivated by this observation, we provide a polynomial-time approximation scheme that recovers a near-optimal signaling policy. Finally, our numerical simulations on semi-synthetic data empirically demonstrate the benefits of using persuasion in the algorithmic recourse setting.

==> approx_new.tex <==
\subsection{An Efficient Approximation Algorithm}\label{sec:approx}
Motivated by the results in Section \ref{sec:regions}, we aim to design a fully polynomial-time approximation scheme to compute an approximately optimal signaling policy for the decision maker. In particular, we sample from $\vTheta$ and solve the empirical analogue of LP \ref{opt:exact}, which provides an $\epsilon$-approximation of the optimal signaling policy with high probability after sampling polynomially-many times. Our method is presented in Algorithm \ref{alg:approx}. Such sampling-based methods are a common approach for constructing approximation algorithms. \citet{dughmi2019algorithmic} provide a similar approximation scheme for the persuasion setting they consider, although their algorithm is not immediately applicable to our algorithmic recourse setting due to differences in how the underlying state of nature affects sender and receiver payoffs. Additionally, their approximation algorithm requires \emph{a priori} knowledge of the true state $\vtheta$, whereas ours does not.

\begin{algorithm}[t]
        \SetAlgoNoLine
        \KwIn{$\vtheta \in \vTheta$, $\epsilon, \delta > 0$}
        \KwOut{Partial signaling policy $\widetilde{\mathcal{S}} := \{p(\sigma = a|R)\}_{\forall a \in \mathcal{A}, R \in \widetilde{\mathcal{R}}}$} 
        Set $K = \left\lceil \frac{1000}{\epsilon^2} \log \left( \frac{4n^2}{\epsilon\delta}\right) \right\rceil$ \\
        Sample $\{\vtheta_1, \ldots, \ldots, \vtheta_K\} \sim \vTheta$.\\
        Let $\widetilde{\mathcal{R}}$ denote the set of observed regions. Compute $\tilde{p}(R)$, $\forall R \in \widetilde{\mathcal{R}}$, where $\tilde{p}(R)$ is the empirical probability that $\vtheta \sim \vTheta \in R$.\\
        Solve the following LP:
        \begin{equation}\label{opt:approx}
        \begin{aligned}
            \max_{p(\sigma = a|R), \forall a \in \mathcal{A}, R \in \widetilde{\mathcal{R}}} \quad &\sum_{a \in \mathcal{A}} \sum_{R \in \widetilde{\mathcal{R}}} \tilde{p}(R) p(\sigma = a|R) u_{dm}(a)\\
            \text{s.t.} \quad &\sum_{R \in \widetilde{\mathcal{R}}} p(\sigma = a|R)\tilde{p}(R)(u_{ds}(a, R) - u_{ds}(a', R) + \epsilon) \geq 0, \; \forall a, a' \in \mathcal{A}\\
            &\sum_{a \in \mathcal{A}} p(\sigma = a|R) = 1, \; \forall R \in \widetilde{\mathcal{R}}, \; \; \;
            p(\sigma = a|R) \geq 0, \; \forall R \in \widetilde{\mathcal{R}}, a \in \mathcal{A}.\\
        \end{aligned}
        \end{equation}
        \caption{Approximation Algorithm for LP \ref{opt:exact}}
        \label{alg:approx}
\end{algorithm}


\vspace{0.2cm}
\noindent \fbox{\parbox{\textwidth}{
\vspace{0.1cm}
\textbf{Signaling policy $\widehat{\mathcal{S}}$}

\vspace{-0.2cm}
\noindent\rule{13.9cm}{0.4pt}
\begin{itemize}[leftmargin=0.65in]
    \item[\textbf{Case 1:}] $\theta \in R$, $R \in \widetilde{\mathcal{R}}$. Recommend an action according to partial signaling policy $\widetilde{\mathcal{S}}$
    \item[\textbf{Case 2:}] $\theta \in R$, $R \not\in \widetilde{\mathcal{R}}$. Recommend action $a^* \in \arg \max_{a \in \mathcal{A}} u_s(a, \vtheta)$ with probability $1$
\end{itemize}
}}
\vspace{0.3cm}

\begin{theorem}\label{thm:approx}
Signaling policy $\widehat{\mathcal{S}}$ can be computed in poly($n, \frac{1}{\epsilon}$) time, is $\epsilon$-BIC, and is $\epsilon$-optimal with probability at least $1 - \delta$.
\end{theorem}

\emph{Proof Sketch.} For the full proof, see Appendix \ref{sec:approx_appendix}. First, we show that Algorithm \ref{alg:approx} runs in poly($n, \frac{1}{\epsilon}$) time, and that $\widehat{\mathcal{S}}$ is an $\epsilon$-BIC signaling policy. Next, we show that if the decision subject follows the recommendations given by $\widehat{\mathcal{S}}$, the expected decision maker utility is at least OPT - $\epsilon$ with probability at least $1 - \delta$ (where OPT is the expected decision maker utility achieved by the optimal signaling policy). In order to do so, we first show that there exists an approximately optimal solution $\mathcal{S}'$ to LP \ref{opt:exact} such that each signal is either (i) \emph{large} (i.e., output with probability above a certain threshold), or (ii) \emph{honest} (i.e., the signal recommends the action the decision subject would take, had they known the true assessment $\vtheta$. We then show that $\mathcal{S}'$ is a feasible solution to LP \ref{opt:approx} with high probability by applying McDiarmid's inequality \cite{mcdiarmid1989method} and a union bound. Finally, we show that this implies that the expected decision maker utility from signaling according to $\widehat{\mathcal{S}}$ is at least OPT $- \epsilon$.

\xhdr{Barriers to exact incentive compatibility}
It is important to note that the signaling policy from Algorithm \ref{alg:approx} is both $\epsilon$-optimal and $\epsilon$-incentive compatible. While one may wonder whether (i) an $\epsilon$-optimal and exactly incentive compatible signaling policy exists, or (ii) an exactly optimal and $\epsilon$-incentive compatible signaling policy exists, \citeauthor{dughmi2019algorithmic} show that this is generally not possible for sampling-based approximation algorithms for Bayesian persuasion. (Note that unlike the other results of \citeauthor{dughmi2019algorithmic}, these results apply directly to the setting we consider.) For completeness, we restate their result below.

\begin{proposition}[\citet{dughmi2019algorithmic}, Theorem 27]
The following hold for every direct sampling-based signaling policy $\mathcal{S}$ for Bayesian persuasion:
\begin{enumerate}
    \item If $\mathcal{S}$ is incentive compatible and $c$-optimal for $c < 1$, then for every integer $K$ there is a distribution $\lambda = \lambda(K)$ on two actions and two states of nature such that the expected number of queries to $\lambda$ made by $\mathcal{S}$ is greater than $K$.
    \item If $\mathcal{S}$ is optimal and $c$-incentive compatible for $c < \frac{1}{4}$, then for every integer $K$ there is a distribution $\lambda = \lambda(K)$ on three actions and three states of nature and a state $\theta$ in the support of $\lambda$ such that the number of queries to $\lambda$ made by $\mathcal{S}$ is greater than $K$.
\end{enumerate}
\end{proposition}

==> computing-new.tex <==
\section{Computing the Optimal Signaling Policy}\label{sec:computing}
In Section \ref{sec:opt}, we show that the problem of determining the decision maker's optimal signaling policy can be transformed from an optimization over infinitely many variables into an optimization over the set of finitely many equivalence regions $\mathcal{R}$ (Theorem \ref{thm:opt}). However, as we show in Appendix \ref{sec:regions}, computing the decision maker's optimal signaling policy by solving \ref{opt:exact} requires reasoning over \emph{exponentially-many} variables, even in relatively simple settings. This motivates the need for a computationally efficient algorithm to approximate \ref{opt:exact}.


We adapt the sampling-based approximation algorithm of \citeauthor{dughmi2019algorithmic} to our setting in order to compute an $\epsilon$-optimal and $\epsilon$-approximate signaling policy in polynomial time, as shown in Algorithm \ref{alg:approx}. At a high level, Algorithm \ref{alg:approx} samples polynomially-many times from the prior distribution over the space of assessment rules, and solves an empirical analogue of \ref{opt:exact}. We show that the resulting signaling policy is $\epsilon$-BIC, and is $\epsilon$-optimal with high probability, for any $\epsilon > 0$.

\begin{algorithm}[t]
        \SetAlgoNoLine
        \KwIn{$\vtheta \in \vTheta$, $\epsilon > 0, \delta > 0$}
        \KwOut{Signaling policy $\widehat{\mathcal{S}} := \{p(\sigma = a|R_{\vtheta})\}_{\forall a \in \mathcal{A}}$ (where  region $R_{\vtheta}$ contains $\vtheta$)} 
        Set $K = \left \lceil \frac{2}{\epsilon^2} \log \left( \frac{2(m^2 + 1)}{\delta}\right) \right \rceil$ \\
        Pick $\ell \in \{1, \ldots, K\}$ uniformly at random. Set $\vtheta_{\ell} = \vtheta$.\\
        Sample $\widetilde{\vTheta} = \{\vtheta_1, \ldots, \vtheta_{\ell-1}, \vtheta_{\ell+1}, \ldots, \vtheta_K\} \sim \pi(\vtheta)$.\\
        Let $\widetilde{\mathcal{R}}$ denote the set of observed regions. Compute $\tilde{p}(R)$, $\forall R \in \widetilde{\mathcal{R}}$, where $\tilde{p}(R)$ is the empirical probability of $\vtheta' \in R$.\\
        Solve
        \small
        \begin{equation}\label{opt:approx}
        \tag*{(APPROX-LP)}
        \begin{aligned}
            \max_{p(\sigma = a|R), \forall a \in \mathcal{A}, R \in \widetilde{\mathcal{R}}} \quad &\sum_{a \in \mathcal{A}} \sum_{R \in \widetilde{\mathcal{R}}} \tilde{p}(R) p(\sigma = a|R) u_{dm}(a)\\
            \text{s.t.} \quad &\sum_{R \in \widetilde{\mathcal{R}}} p(\sigma = a|R)\tilde{p}(R)(u_{ds}(a, R) - u_{ds}(a', R) + \epsilon) \geq 0, \; \forall a, a' \in \mathcal{A}\\
            &\sum_{a \in \mathcal{A}} p(\sigma = a|R) = 1, \; \forall R \in \widetilde{\mathcal{R}}, \; \; \;
            p(\sigma = a|R) \geq 0, \; \forall R \in \widetilde{\mathcal{R}}, a \in \mathcal{A}.\\
        \end{aligned}
        \end{equation}
        \normalsize
        Return signaling policy $\widehat{\mathcal{S}} := \{p(\sigma = a|R_{\vtheta})\}_{\forall a \in \mathcal{A}}$.\\
        \caption{Approximation Algorithm for \ref{opt:exact}}
        \label{alg:approx}
\end{algorithm}


\begin{theorem}\label{thm:approx}
Algorithm \ref{alg:approx} runs in poly($m, \frac{1}{\epsilon}$) time (where $m = |\mathcal{A}|$), and implements an $\epsilon$-BIC signaling policy that is $\epsilon$-optimal with probability at least $1 - \delta$.
\end{theorem}

See Appendix \ref{sec:approx_appendix} for the full proof.


\iffalse
%\noindent \xhdr{Barriers to exact optimality and incentive compatibility}
\noindent \xhdr{Bi-criteria approximation}
It is important to note that the signaling policy from Algorithm \ref{alg:approx} is both $\epsilon$-optimal and $\epsilon$-incentive compatible. While one may wonder whether (i) an $\epsilon$-optimal and exactly incentive compatible signaling policy exists, or (ii) an exactly optimal and $\epsilon$-incentive compatible signaling policy exists, \citeauthor{dughmi2019algorithmic} show that this is generally not possible for sampling-based approximation algorithms for Bayesian persuasion (see Theorem 27 in \citet{dughmi2019algorithmic}). Note that unlike the other results in \citet{dughmi2019algorithmic}, these results directly apply to the setting we consider. 
\fi 

\noindent \xhdr{Computational complexity} 
Recall that the algorithm for computing the optimal policy runs in time polynomial in the number of equivalence regions $|\mathcal{R}|$, which can scale exponentially in the number of actions $m$. However, without any structural assumptions, the input prior over the space of assessment rules $\vTheta$ can scale exponentially in the number of features $d$. When $m$ and $d$ are comparable, our algorithm runs in time polynomial in the input size. We leave open the question of whether there are classes of succinctly represented prior distributions that permit efficient algorithms for computing the optimal policy in time polynomial in $d$ and $m$. It is also plausible to design efficient algorithms that only require some form of query access to the prior distribution. However, the information-theoretic lower bounds of \cite{dughmi2019algorithmic} rule out the query access through sampling, as they show that no sampling-based algorithm can compute the optimal signaling policy with finite samples across all problem instances. 

This suggests that in order to compute the optimal signaling policy that satisfies exact BIC constraints, an algorithm must take the entire prior over $\vTheta$ as input. Without making any assumptions on the specific form of the prior, the representation of the prior will have size that is exponential in the number of observable features. In this case, we expect the running time of an algorithm which takes the prior as input to be exponential in the number of features as well. 

==> computing.tex <==
\section{Computing the Optimal Signaling Policy}\label{sec:computing}
In Section \ref{sec:opt}, we show that the problem of determining the decision maker's optimal signaling policy can be transformed from an optimization over infinitely many variables into an optimization over the set of finitely many equivalence regions $\mathcal{R}$ (Theorem \ref{thm:opt}). However, as we will show in Section \ref{sec:regions}, computing the decision maker's optimal signaling policy by solving \ref{opt:exact} requires reasoning over \emph{exponentially-many} variables, even in relatively simple settings. This motivates the need for a computationally efficient algorithm to approximate \ref{opt:exact}, which we present in Section \ref{sec:approx}.

\subsection{Computational Barriers}\label{sec:regions}
In this section, we show that even in the setting where each action only affects one observable feature (e.g., as shown in Figure \ref{fig:actionscheme}), the number of equivalence regions in \ref{opt:exact} is still exponential in the size of the input. 
%See Figure 1 for a graphical representation of such a setting.
While somewhat simplistic, we believe this action scheme reasonably reflects real-world settings in which the decision subjects are under time or resource constraints when deciding which action to take. For example, the decision subject may need to choose between paying off some amount of debt and opening a new credit card when strategically modifying their observable features before applying for a loan.


\usetikzlibrary{positioning}
\tikzset{main node/.style={circle,draw,minimum size=1cm,inner sep=0pt, thick},}
\begin{figure}
    \centering
    %\resizebox{0.45\textwidth}{!}{%
      \begin{tikzpicture}

    \begin{scope}[xshift=4cm]
    \node[main node] (1) {$a_{i,1}$};
    \node[main node] (2) [above = 0.5cm  of 1]  {$a_{d,1}$};
    \node[main node] (3) [left = 1cm  of 1] {$a_{\emptyset}$};
    \node[main node] (4) [below = 0.5cm  of 1] {$a_{1,1}$};
    \node[main node] (5) [right = 1.5cm  of 4] {...};
    \node[main node] (6) [right = 1.5cm  of 5] {$a_{1,m_1}$};
    \node[main node] (7) [right = 1.5cm  of 1] {...};
    \node[main node] (8) [right = 1.5cm  of 7] {$a_{i,m_i}$};
    \node[main node] (9) [right = 1.5cm  of 2] {...};
    \node[main node] (10) [right = 1.5cm  of 9] {$a_{d,m_d}$};
    \node at (1,1) {\rotatebox{90}{{...}}};
    \node at (1,-1) {\rotatebox{90}{{...}}};
    % \node at (1,0.75) {...};
    \path[draw,thick]
    (3) edge node {} (4)
    (3) edge node {} (1)
    (3) edge node {} (2)
    (4) edge node {} (5)
    (5) edge node {} (6)
    (1) edge node {} (7)
    (7) edge node {} (8)
    (2) edge node {} (9)
    (9) edge node {} (10)
    ;
    \end{scope}
\end{tikzpicture}
%}
    \caption{Graphical representation of special ordering over the actions available to each decision subject. Each branch corresponds to an observable feature and each node corresponds to a possible action the decision subject may take. The root corresponds to taking no action (denoted by $a_{\emptyset}$). Nodes further away from the root on branch $i$ correspond to higher $\Delta \vx_i$, i.e., $\Delta \vx_i(a_{\emptyset}) \prec \Delta \vx_i(a_{i,1}) \prec \ldots \prec \vx_i(a_{i,m_i})$.}
  \label{fig:actionscheme}
\end{figure}




% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{treerotate.png}
%     \caption{Graphical representation of special ordering over the actions available to each decision subject. Each branch corresponds to an observable feature and each node corresponds to a possible action the decision subject may take. The root corresponds to taking no action (denoted by $a_{\emptyset}$). Nodes further away from the root on branch $i$ correspond to higher $\Delta \vx_i$, i.e., $\Delta \vx_i(a_{\emptyset}) \prec \Delta \vx_i(a_{i,1}) \prec \ldots \prec \Delta \vx_i(a_{i,m_i})$.}
%     \label{fig:actionscheme}
% \end{figure}
\iffalse
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
  \includegraphics[scale=0.4]{simpletree.png}
  \caption{Graphical representation of special ordering over the actions available to each decision subject. Each branch corresponds to an observable feature and each node corresponds to a possible action the decision subject may take. The root corresponds to taking no action (denoted by $a_{\emptyset}$). Nodes further away from the root on branch $i$ correspond to higher $\Delta \vx_i$, i.e., $\Delta \vx_i(a_{\emptyset}) \prec \Delta \vx_i(a_{i,1}) \prec \ldots \prec \vx_i(a_{i,m_i})$.}
  \label{fig:actionscheme}
\end{wrapfigure}
\fi 

Under this setting, \ref{opt:exact} optimizes over $\Theta(m|\mathcal{R}|)$ variables, where $m$ is the number of actions available to each agent and $|\mathcal{R}|$ is the number of equivalence regions. In order to determine the size of $\mathcal{R}$, we note that an equivalence region can be alternatively characterized by observing that assessment rules $\vtheta$ and $\vtheta'$ belong to the same equivalence region if the difference in their predictions for any two actions $a$ and $a'$ is the same. (This follows from straightforward algebraic manipulation of Definition \ref{def:region}.) As such, an equivalence region $R$ can essentially be characterized by the set of actions $A_R \subseteq \mathcal{A}$ which receive a positive classification when $\vtheta \in R$.\footnote{Specifically, if taking action $a$ results in a positive classification for some $\vtheta \in \vTheta$ and a negative classification for $\vtheta \in \vTheta$, the only way for $\vtheta$ and $\vtheta'$ to be in the same equivalence region is if taking \emph{any} action in $\mathcal{A}$ results in a positive classification for $\vtheta$ and a negative classification for $\vtheta'$. Besides this special case, if $\vtheta$ and $\vtheta'$ result in different classifications for the same action, they are in different equivalence regions.}

%In order to determine the size of $\mathcal{R}$, we make use of an alternative characterization of a region of $\vTheta$ below, which can be derived by algebraic manipulation of Definition \ref{def:region}.

\iffalse
\begin{definition}[Region, revisited]\label{def:region-alt}
A region $R$ of $\vTheta$ is the set of all $\vtheta \in \vTheta$ such that $\hat{y}(\vtheta, a) - \hat{y}(\vtheta, a') = \hat{y}(\vtheta', a) - \hat{y}(\vtheta', a')$, where we abuse notation by defining $\hat{y}(\vtheta, a) := \text{sign}\{(\vx_0 + \Delta \vx(a))^\top \vtheta\}$.
%$\text{sign}\{(\vx_0 + \Delta \vx(a))^\top \vtheta + b\} - \text{sign}\{(\vx_0 + \Delta \vx(a'))^\top \vtheta + b\} = \text{sign}\{(\vx_0 + \Delta \vx(a))^\top \vtheta' + b'\} - \text{sign}\{(\vx_0 + \Delta \vx(a'))^\top \vtheta' + b'\}$, $\forall a, a' \in \mathcal{A}$, $(\vtheta,b), (\vtheta',b') \in R$.
\end{definition}
\fi 

%In other words, assessments $\vtheta$ and $\vtheta'$ belong to the same region if the difference in their predictions for any two actions $a$ and $a'$ is the same. An immediate consequence of this alternative definition is that a region $R$ can essentially be uniquely characterized by the set of actions $A_R \subseteq \mathcal{A}$ which receive a positive classification when $\vtheta \in R$.
%\footnote{Specifically, if taking action $a$ results in a positive classification for some $\vtheta \in \vTheta$ and a negative classification for $\vtheta \in \vTheta$, the only way for $\vtheta$ and $\vtheta'$ to be in the same region is if taking \emph{any} action in $\mathcal{A}$ results in a positive classification for $\vtheta$ and a negative classification for $(\vtheta', b')$. Besides this special case, if $\vtheta$ and $\vtheta'$ result in different classifications for the same action, they are in different regions by Definition \ref{def:region-alt}.} 
Armed with this new characterization of an equivalence region, we are now ready to show the scale of $|\mathcal{R}|$ for the setting described in Figure \ref{fig:actionscheme}. 

\begin{prop}\label{prop:exp}
For the setting described in Figure \ref{fig:actionscheme}, there are $|\mathcal{R}| = \Pi_{i=1}^d m_i - 1$ equivalence regions, where $d$ is the number of observable features of the decision subject and $m_i$ ($\forall i \in [d]$) is the number of actions the decision subject has at their disposal to improve observable feature $i$.
\end{prop}

\begin{proof}
In order to characterize the number of equivalence regions $|\mathcal{R}|$, we define the notion of a \emph{dominated} action $a$, where an action $a$ is dominated by some other action $a'$ if $\Delta \vx(a) \preceq \Delta \vx (a')$, with strict inequality holding for at least one index. Using this notion of dominated actions and our refined characterization of an equivalence region, it is straightforward to see that if action $a$ is dominated by action $a'$, then  $a' \in A_R$ for any equivalence region $R$ where $a \in A_R$. Proposition \ref{prop:exp} then follows directly from the fact that each action only affects one observable feature.
\iffalse
\begin{definition}[Dominated Action]\label{def:dominated}
An action $a$ is dominated by some other action $a'$ if $\Delta \vx(a) \preceq \Delta \vx (a')$ and $\Delta \vx_i(a) < \Delta \vx_i(a')$ for at least one index $i \in \{1, \ldots, d\}$. 
\end{definition}
\fi 
%For example, in Figure \ref{fig:actionscheme}, action $a_{i,j}$ is dominated by action $a_{i,k}$, $\forall i, 1 \leq j < k \leq m_i$. Note that in general if action $a'$ dominates action $a$, then it is always possible to write $\Delta \vx_i(a')$ in terms of $\Delta \vx_i(a)$, i.e., $\Delta \vx_i(a') = \Delta \vx_i(a) + \boldsymbol{\delta}(a,a')$, where $\boldsymbol{\delta}(a,a') \succeq \mathbf{0}_d$ and $\delta_{i}(a,a') > 0$ for some $i \in \{1, \ldots, d\}$.
\iffalse
\begin{lemma}\label{lem:dom}
If action $a$ is dominated by action $a'$, then  $a' \in A_R$ for any equivalence region $R$ where $a \in A_R$.
\end{lemma}
\begin{proof}
The decision subject receives a positive classification for some $\vtheta \in \vTheta$ if $(\vx_0 + \Delta \vx(a))^\top \vtheta \geq 0$.
If $a'$ dominates $a$, then $\Delta \vx(a')$ can be written as $\Delta \vx(a') = \Delta \vx(a) + \boldsymbol{\delta}(a,a')$, where $\boldsymbol{\delta}(a,a') \succeq \mathbf{0}_d$. Therefore, if $(\vx_0 + \Delta \vx(a))^\top \vtheta \geq 0$ (i.e., when $a \in A_R$), then $(\vx_0 + \Delta \vx(a'))^\top \vtheta  = (\vx_0 + \Delta \vx(a))^\top \vtheta + \boldsymbol{\delta}(a,a')^\top \vtheta \geq 0$ (and $a' \in A_R$), since $\boldsymbol{\delta}(a,a') \succeq \mathbf{0}_d$ and $\vtheta \in \mathbb{R}^d_+$.
\end{proof}
\fi 
\end{proof}

%Under this setting, when the number of observable features $d$ is small, the decision maker can essentially be thought of as optimizing over a number of variables that is polynomial in the number of actions $m$. However, as $d$ grows large, LP \ref{opt:approx} quickly becomes intractable.

%Now that the space of regions $\mathcal{R}$ is specified, it is possible to calculate $\pi(R)$ for $R \in \mathcal{R}$, given $\pi(\vtheta, b)$ without enumerating all possibilities. Recall that a region $R$ is characterized by the set of actions $A_R \subseteq \mathcal{A}$ that receive a positive classification whenever $(\vtheta, b) \in R$. Each action $a \in \mathcal{A}$ is associated with a hyperplane in $\vTheta$-space, $(\vx_0 + \Delta \vx(a))^\top \vtheta + b = 0$. The decision subject receives a positive classification when taking action $a$ for all $(\vtheta, b)$ such that $(\vx_0 + \Delta \vx(a))^\top \vtheta + b \geq 0$ and a negative classification otherwise. Therefore, each region $R$ is a convex subspace of $\vTheta$ , and can be calculated as
%    $\pi(R) = \int_{(\vtheta, b) \in R} \pi(\vtheta, b) dR$.

Proposition \ref{prop:exp} {shows that} the computation of \ref{opt:exact} quickly becomes intractable as the number of observable features grows large, even in this relatively simple setting. This motivates the need for an approximation algorithm for \ref{opt:exact}, which we present in Section \ref{sec:approx}.
    
%\input{approx_new}
\input{approx_old}

==> extensions.tex <==
\section{Extensions}\label{sec:extensions}


==> joint_optimization.tex <==
\section{Extension: Joint Optimization over Decision Rule \& Signaling Policy}
\begin{equation}\label{opt:joint}
\begin{aligned}
    \max_{p(\vtheta'_i), p(\sigma = a|\vtheta'_i), \forall a \in \mathcal{A}, i \in [N]} \quad &\sum_{i=1}^N \sum_{a \in \mathcal{A}} p(\vtheta'_i) p(\sigma = a|\vtheta'_i) u_{dm}(a)\\
    \text{s.t.} \quad &\sum_{i=1}^N p(\sigma = a|\vtheta'_i) p(\vtheta'_i) (u_{ds}(a, \vtheta'_i) - u_{ds}(a', \vtheta'_i)) \geq 0, \; \forall a, a' \in \mathcal{A}\\
    &\sum_{a \in \mathcal{A}} p(\sigma = a|\vtheta'_i) = 1, \; \forall i \in [N], \; \; \;
    p(\sigma = a|\vtheta'_i) \geq 0, \; \forall i \in [N], a \in \mathcal{A}\\
    &\sum_{i=1}^N p(\vtheta'_i) = 1, \;\;\; p(\vtheta'_i) \geq 0, \; \forall i \in [N]\\
\end{aligned}
\end{equation}

\begin{theorem} 
If $\{\vtheta'_i\}_{i=1}^N = \{\vtheta'_R\}_{R \in \mathcal{R}}$, where $N = |\mathcal{R}|$, $\vtheta'_R \in R$, $\forall R \in \mathcal{R}$, then 
\begin{equation*}
    \sum_{i=1}^N \sum_{a \in \mathcal{A}} p(\vtheta'_i) p(\sigma = a|\vtheta'_i) u_{dm}(a) = u^*,
\end{equation*}
where $u^*$ is the maximum possible expected decision-maker utility over $\Delta(\vTheta, \mathcal{A})$ and $\{(p(\vtheta'_i), \{p(\sigma = a| \vtheta_i'\}_{a \in \mathcal{A}}) \}_{i=1}^N$ is the solution to LP \ref{opt:joint}.
\end{theorem}

\begin{proof}

\end{proof}

==> model.tex <==
\section{Optimal Signaling Policy}\label{sec:opt}

% While our example signaling policy in the previous section leads to higher expected decision maker utility, there is no reason \emph{a priori} to believe it is optimal, or that 

In Section~\ref{sec:ex}, we show a one-dimensional setting, where a signaling policy can obtain unbounded better utilities compared to revealing full information and revealing no information. We now derive the decision maker's optimal signaling policy for the general setting with arbitrary numbers of observable features and actions described in Section \ref{sec:background}. Under the general setting, the decision maker's optimal signaling policy can be described by the following optimization:
\small
\begin{equation}\label{eqn:opt}
\begin{aligned}
    &\max_{p(\sigma = a|\vtheta), \forall a \in \mathcal{A}} \quad \mathbb{E}_{\sigma \sim \mathcal{S}, \vtheta \sim \Pi}[u_{dm}(\sigma)]\\
    \text{s.t.} \quad &\mathbb{E}_{\vtheta \sim \Pi}[u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta) | \sigma = a] \geq 0, \; \forall a, a' \in \mathcal{A},
\end{aligned}
\end{equation}
\normalsize
where we omit the valid probability constraints over $p(\sigma = a|\vtheta), a \in \mathcal{A}$ for brevity. In words, the decision maker wants to design a signaling policy $\mathcal{S}$ in order to maximize their expected utility, subject to the constraint that the signaling policy is BIC. At first glance, the optimization may initially seem hopeless as there are infinitely many values of $p(\sigma = a|\vtheta)$ (one for every possible $\vtheta \in \vTheta$) that the decision maker's optimal policy must optimize over. However, we will show that the decision maker's optimal policy can actually be recovered by optimizing over finitely many variables. 

By rewriting the BIC constraints as integrals over $\vTheta$ and applying Bayes' rule, our optimization over $p(\sigma = a|\vtheta), a \in \mathcal{A}$ takes the following form
\small
\begin{equation*}
\begin{aligned}
    &\max_{p(\sigma = a|\vtheta), \forall a \in \mathcal{A}} \quad \mathbb{E}_{\sigma \sim \mathcal{S}, \vtheta \sim \Pi}[u_{dm}(\sigma)]\\
    \text{s.t.} \quad &\int_{\vTheta} p(\sigma = a|\vtheta)\pi(\vtheta)(u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta)) d\vtheta \geq 0, \; \forall a, a' \in \mathcal{A}.
\end{aligned}
\end{equation*}
\normalsize

Note that if $u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta)$ is the same for some ``equivalence region'' $R \subseteq \vTheta$ (which we formally define below), we can pull $u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta)$ out of the integral and instead sum over the different equivalence regions. Intuitively, an equivalence region can be thought of as the set of all $\vtheta \in \vTheta$ pairs that are indistinguishable from a decision subject's perspective because they lead to the exact same utility for any possible action the decision subject could take.
Based on this idea, we formally define a region of $\vTheta$ as follows. 

\begin{definition}[Equivalence Region]\label{def:region}
Two assessments $\vtheta, \vtheta'$ are \emph{equivalent} (w.r.t. $u_{ds}$) if $u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta) = u_{ds}(a, \vtheta') - u_{ds}(a', \vtheta')$, $\forall a, a' \in \mathcal{A}$. An \emph{equivalence region} $R$ is a subset of $\vTheta$ such that for any $\theta \in R$, all $\theta'$ equivalent to $\theta$ are also in $R$. We denote the set of all equivalence regions by $\mathcal{R}$.
% is the set of all $\vtheta \in \vTheta$ such that 
% $u_{ds}(a, \vtheta) - u_{ds}(a', \vtheta) = u_{ds}(a, \vtheta') - u_{ds}(a', \vtheta')$, $\forall a, a' \in \mathcal{A}$, $\vtheta, \vtheta' \in R$. 
\end{definition}

\iffalse
In Figure \ref{fig:region}, we show an example of how different equivalence regions might partition the space of possible assessment rules $\vTheta$. In this example, there are two actions and two observable features, and the space of $\vTheta$ is partitioned into three different equivalence regions. Note that as long as the set of actions $\mathcal{A}$ is finite, $|\mathcal{R}| < \infty$. 
\fi 
After pulling the decision subject utility function out of the integral, our optimization takes the following form:

\iffalse
\begin{figure}[t]
    \centering
    %\resizebox{0.4\textwidth}{!}{%
      \begin{tikzpicture}[scale=1.5,extended line/.style={shorten >=-#1,shorten <=-#1},every text node part/.style={align=center}]
% \draw grid (4,2);
\draw[draw=black] (0,0) rectangle ++(1,1);
\draw[draw=black] (1,0) rectangle ++(3,1);
\draw[draw=black] (0,1) rectangle ++(1,1);
\draw[draw=black] (1,1) rectangle ++(3,1);
\draw [->](0,0)--(0,2.2) node[right]{$\theta_2$};
\draw [->](0,0)--(4.2,0) node[right]{$\theta_1$};
\foreach \x/\xtext in {0, 1/\frac{1}{2}, 4/2}
{\draw (\x cm,1pt ) -- (\x cm,-1pt ) node[anchor=north] {$\xtext$};}
\foreach \y/\ytext in {1/\frac{1}{2}, 2/1}
{\draw (1pt,\y cm) -- (-1pt ,\y cm) node[anchor=east] {$\ytext$};}
\node at (0.5,0.5) {$R_0$\\ $\{\emptyset\}$};
\node at (2.5,0.5) {$R_1$\\ $\{a_1\}$};
\node at (2.5,1.5) {$R_0$\\ $\{a_1,a_2\}$};
\node at (0.5,1.5) {$R_2$\\ $\{a_2\}$};
\end{tikzpicture}%}
\caption{An illustration of the equivalence regions for a two action ($a_1$, $a_2$) and two observable feature ($x_1, x_2$) setting, where $\vTheta = [0, 2] \times [0, 1] \times \{\frac{1}{2}\}$. Consider an individual with $\vx_0 = [0, 0, 1]^\top$, $\Delta \vx(a_1) = [1, 0, 0]^\top$, and $\Delta \vx(a_2) = [0, 1, 0]^\top$. The equivalence regions of $\vTheta$ are quadrants described the set of actions the decision subject could take in order to receive a positive classification. Region $R_0$ contains the bottom-left and top-right quadrants of $\vTheta$, region $R_1$ contains the bottom-right quadrant of $\vTheta$, and region $R_2$ contains the top-left quadrant of $\vTheta$.}
  \label{fig:region}
\end{figure}
\fi 

\small
\begin{equation*}
\begin{aligned}
    \max_{p(\sigma = a|\vtheta), \forall a \in \mathcal{A}} \quad &\mathbb{E}_{\sigma \sim \mathcal{S}, \vtheta \sim \Pi}[u_{dm}(\sigma)]\\
    \text{s.t.} \quad &\sum_{R \in \mathcal{R}} (u_{ds}(a, R) - u_{ds}(a', R)) \int_{\vtheta \in R} p(\sigma = a|\vtheta)\pi(\vtheta) d\vtheta \geq 0, \; \forall a, a' \in \mathcal{A}.\\
\end{aligned}
\end{equation*}
\normalsize


Now that the decision subject's utility $u_{ds}(\cdot)$ no longer depends on $\vtheta$, we can integrate $p(\sigma = a|\vtheta) \pi(\vtheta)$ over each equivalence region $R$. We denote $p(R)$ as the probability that the true $\vtheta \in R$ according to the prior.

\small
\begin{equation*}
\begin{aligned}
    \max_{p(\sigma = a|R), \forall a \in \mathcal{A}, R \in \mathcal{R}} \quad &\mathbb{E}_{\sigma \sim \mathcal{S}, \theta \sim \Pi}[u_{dm}(\sigma)]\\
    \text{s.t.} \quad &\sum_{R \in \mathcal{R}} p(\sigma = a|R) \pi(R)(u_{ds}(a, R) - u_{ds}(a, R)) \geq 0, \; \forall a, a' \in \mathcal{A}.\\
\end{aligned}
\end{equation*}
\normalsize

Since it is possible to write the constraints in terms of $p(\sigma = a|R)$, $\forall a \in \mathcal{A}, R \in \mathcal{R}$, it suffices to optimize directly over these quantities. The final step is to rewrite the objective. For completeness, we include the constraints which make each $\{p(\sigma = a_1|R), p(\sigma = a_2|R), \ldots, p(\sigma = a_m|R)\}$, $\forall R$ a valid probability distribution.

\begin{theorem}[Optimal signaling policy]\label{thm:opt}
The decision maker's optimal signaling policy can be characterized by the following linear program OPT-LP:
\small
\begin{equation}\label{opt:exact}
\tag*{(OPT-LP)}
\begin{aligned}
    \max_{p(\sigma = a|R), \forall a \in \mathcal{A}, R \in \mathcal{R}} \quad &\sum_{a \in \mathcal{A}} \sum_{R \in \mathcal{R}} p(R) p(\sigma = a|R) u_{dm}(a)\\
    \text{s.t.} \quad &\sum_{R \in \mathcal{R}} p(\sigma = a|R)p(R)(u_{ds}(a, R) - u_{ds}(a', R)) \geq 0, \; \forall a, a' \in \mathcal{A}\\
    &\sum_{a \in \mathcal{A}} p(\sigma = a|R) = 1, \; \forall R, \; \; \;
    p(\sigma = a|R) \geq 0, \; \forall R \in \mathcal{R}, a \in \mathcal{A},\\
\end{aligned}
\end{equation}
\normalsize
\end{theorem}

where $p(\sigma = a|R)$ denotes the probability of sending recommendation $\sigma = a$ if $\vtheta \in R$.
Note that the linear program OPT-LP is always feasible, as the decision maker can always recommend the action the decision subject would play according to the prior, which is BIC.
